Faster Approximation Schemes for Fractional Multicommodity Flow Problems via Dynamic Graph Algorithms

We combine the work of Garg and Konemann, and Fleischer with ideas from dynamic graph algorithms to obtain faster (1-eps)-approximation schemes for various versions of the multicommodity flow problem. In particular, if eps is moderately small and the size of every number used in the input instance is polynomially bounded, the running times of our algorithms match - up to poly-logarithmic factors and some provably optimal terms - the Omega(mn) flow-decomposition barrier for single-commodity flow.

==> acknowledgments.tex <==
\section*{Acknowledgments}

We are grateful to Michel Goemans, Debmalya Panigrahi, and anonymous reviewers for helpful comments. We also thank Lisa Fleischer, and David Shmoys for providing useful references. 

